Learning to Select Context in a Hierarchical and Global Perspective for Open-domain Dialogue Generation

Open-domain multi-turn conversations mainly have three features, which are hierarchical semantic structure, redundant information, and long-term dependency. Grounded on these, selecting relevant context becomes a challenge step for multi-turn dialogue generation. However, existing methods cannot differentiate both useful words and utterances in long distances from a response. Besides, previous work just performs context selection based on a state in the decoder, which lacks a global guidance and could lead some focuses on irrelevant or unnecessary information. In this paper, we propose a novel model with hierarchical self-attention mechanism and distant supervision to not only detect relevant words and utterances in short and long distances, but also discern related information globally when decoding. Experimental results on two public datasets of both automatic and human evaluations show that our model significantly outperforms other baselines in terms of fluency, coherence, and informativeness.

==> relatedwork.tex <==
\section{Related Work}

For multi-turn conversations, there are two branches of research to obtain an appropriate response for the given context, which are response selection and response generation.

\subsection{Response Selection}
The task of response selection aims to choose an appropriate response from several given candidates. \newcite{lowe2015ubuntu} and \newcite{zhou2016multi} represent the context and response as two semantic vectors (the last hidden states of RNNs) and then measure their relevance to select the proper response. \newcite{wu2017sequential} propose the sequential matching network (SMN) to take the hidden state at each time step as a text segment representation, and measure the distance between context and response via segment-segment matching matrices. \newcite{zhang2018modeling} introduce self-matching attention to better model the dependency among context utterances. \newcite{zhou2018multi} construct representations of text segments at different granularities with stacked self-attention, and extract the truly matched segment pairs with attention across the context and response. 

\subsection{Response Generation}
Apart from response selection, some researchers try to generate a response from scratch, which is not constrained by those given candidates and can also be customized. Intuitively, it is not reasonable to just consider utterances in the context as a concatenated long sequence \cite{yan2016learning,sordoni2015neural}. Therefore, hierarchical models play an important role in this field. \newcite{serban2016building} propose the hierarchical recurrent encoder-decoder (HRED) model with a context RNN to integrate previous information from traditional utterance RNNs. To capture utterance-level variations, \newcite{serban2017hierarchical} raise a new model, Variational HRED (VHRED), that augments HRED with conditional variational autoencoder (CVAE). After that, VHCR \cite{park2018hierarchical} adds a conversation-level latent variable on top of VHRED, while CSRR \cite{shen2019modeling} uses three-hierarchy latent variables to model the complex dependency among utterances. In order to detect relevant contextual utterances, \newcite{tian2017make} and \newcite{zhang2018context} apply cosine similarity and attention mechanism, respectively, between representations of each utterance and the query under the assumption that the query is most related to the response. HRAN \cite{xing2018hierarchical} combines the attention results at both word level and utterance level. Besides, HVMN \cite{chen2018hierarchical} and ReCoSa \cite{zhang2019recosa} try to solve the long-term dependency of utterances in multi-turn conversations with the assistance of either memory networks or self-attention mechanism. \newcite{bak2019variational} integrate user information to improve the performance of VHCR.

Our work is different from the above in following aspects: (1) We use the hierarchical self-attention mechanism to not only detect relevant information at both word and utterance levels but also model the entire conversation structure. (2) We propose a globally distant supervision to guide the response generation process, that is, using the utterance-level similarity information with high-quality pre-trained sentence-embedding models at each decoding step. 


